On the Nonlinear Eshelby Inclusion Problem and its Isomorphic Growth Limit

In the late 1950's, Eshelby's linear solutions for the deformation field inside an ellipsoidal inclusion and, subsequently, the infinite matrix in which it is embedded were published. The solutions' ability to capture the behavior of an orthotropically symmetric shaped inclusion made it invaluable in efforts to understand the behavior of defects within, and the micromechanics of, metals and other stiff materials throughout the rest of the 20th century. Over half a century later, we wish to understand the analogous effects of microstructure on the behavior of soft materials; both organic and synthetic; but in order to do so, we must venture beyond the linear limit, far into the nonlinear regime. However, no solutions to these analogous problems currently exist for non-spherical inclusions. In this work, we present an accurate semi-inverse solution for the elastic field in an isotropically growing spheroidal inclusion embedded in an infinite matrix, both made of the same incompressible neo-Hookean material. We also investigate the behavior of such an inclusion as it grows infinitely large, demonstrating the existence of a non-spherical asymptotic shape and an associated asymptotic pressure. We call this the isomorphic limit, and the associated pressure the isomorphic pressure.

==> Chapter4del.tex <==
\section{Ellipsoids with Analytically Described Fields}
In the following sections we futher restrict ourselves to the study of two particular ellipsoids: spheroids ($A_1=A_2$) and elliptic cylinders ($A_3\to\infty$). For these ellipsoids we find that the form of the elastic fields are analytically tractable, subject to energy minimization of the form of equation (\ref{eq:minimizationConditions}).



% \subsection{Elliptic Cylinders ($A_3\to\infty$)}
% \begin{subequations}
% For the case of an elliptic cylinder we assume that $\hat\Phi_3(\Lambda)=\hat\varphi_3(\Lambda)=\infty$. Similarly to the case of the spheroid, we are left with a single finite aspect ratio $\Phi_2$ in the reference configuration, and $\varphi_2$ in the deformed configuration. For simplicity in the section on spheroids we will drop the subscript "2" in the following section. That is to say that $\{\Phi_2,\Phi_{02},\Phi_{\infty 2},\varphi_2, \varphi_{02}, \gamma_2\}\equiv\{\Phi,\Phi_{0},\Phi_{\infty},\varphi, \varphi_{0}, \gamma\}$. As such (\ref{eq:RefEllipsoids}) reduces to:
% \begin{equation}
%     X_1^2+\frac{X_2^2}{\Phi^2}=A_1^2\Lambda^2\;.
% \end{equation}

% In the linear limit it can be shown that the set of confocal elliptical cylinders including $\partial\mathcal{D}_I^0$ are transformed to a new set of ellipses in the deformed configuration for any \emph{2D isotropic eigenstrain} in the $\e_1$-$\e_2$ plane (any diagonal $\F^*$ with $F^*_{11}=F^*_{22}$) regardless of the value of $F^*_{33}$. Therefore, going forward we will consider the case of \emph{2D isotropic planar transformations} as the simplest of such cases, such that:
% \begin{equation}\label{eq:2DGrowth}
%     \F^* = \lambda^*\;(\e_1\otimes\e_1) + \lambda^*\;(\e_2\otimes\e_2) + (\e_3\otimes\e_3)\;.
% \end{equation}
% In this case, in the linear limit, we find that the resulting deformation from such a transformation satisfies with transformation in the $\e_3$ direction satisfies the plane strain condition ($F_{33}=F^*_{33}=F^e_{33}=1$) and thus we will make the kinematic assumption that our nonlinear solution will also remain in plane strain. This implies that (\ref{eq:xofX}) becomes:
% \begin{equation} \label{eq:xofXSum2D}
%     \x = \Chi(\X) = \left\{\frac{\alpha}{\Lambda}X_1,\;\frac{\varphi\alpha}{\Phi\Lambda}X_2,\;X_3\right\}.
% \end{equation}

% In the following calculations extrinsic quantities (volume, total free energy, free energy per unit reference volume, etc.) will now refer to their value per unit depth in the $\e_3$ direction. For instance (\ref{eq:VolumeInclusion})
% becomes:
% \begin{equation}
%     V^0 = \pi A_1A_2 = \pi\Phi_0 A_1^2\;,
% \end{equation}
% where $V^0$ is the volume of $\mathcal{D}_I^0$ per unit depth in the $\e_3$ direction and (\ref{eq:VolumeDefInclusion}) becomes:
% \begin{equation}\label{eq:VolumeDefInclusion2D}
%     V^* = \pi a_1a_2 = J^*_IV^0\;,
% \end{equation}
% where $J^*_I = (\lambda^*)^2$ and $V^*$ is now the volume of $\mathcal{D}_I$ per unit depth in the $\e_3$ direction.
% \end{subequations}

% The following is a summary of the equations which can be used to solve for the field in a elliptic cylindrical inclusion and the surrounding matrix during 2D isotropic planar transformations, given our kinematic assumptions and choosing the generalized version of the undeformed aspect ratio function (\ref{eq:PhiGj}). Detailed derivations of these equations can be found in Appendix B. The deformation $\Chi(\X)$ can be described via the following functions for the undeformed aspect ratio: 
% \begin{subequations}
%     \begin{equation}\label{eq:PhiMatCylinder}
%         \hat\Phi(\Lambda)=
%         \begin{cases}
%             \Phi_{0}, & 0<\Lambda< 1 \\
%              \displaystyle\frac{\sqrt{(\Phi_{0}^2-\Phi_{\infty }^2)+\Phi_{\infty }^2\Lambda^2}}{\Lambda}, & \Lambda>1\;,
%         \end{cases}
%     \end{equation}
%  and the corresponding deformed radial parameter $\alpha$:
%     \begin{equation}\label{eq:alphaMatCylinder}
%         \hat\alpha(\Lambda)=
%         \begin{dcases}
%             \lambda^*\left(\frac{\Phi_{0}}{\varphi_{0}}\right)^{\frac{1}{2}}\Lambda, & 0<\Lambda< 1 \\
%             S\left(\frac{\Phi\Lambda^{2}+\dV}{\f}\right)^{\frac{1}{2}}\;, & \Lambda>1\;,
%         \end{dcases}
%     \end{equation}
% where:
%     \begin{equation}
%         S=\hat{S}(\Lambda)=\left(\frac{\left(\xi-2\dV \f\right)\left(\Phi\xi+\dV \left(\Phi^{2}+\f^{2}\right)\right)\left((\Phi^2+\f^{2})\Lambda^{2}-\xi\right)}{\left(\xi+2\dV \f\right)\left(\Phi\xi-\dV \left(\Phi^{2}+\f^{2}\right)\right)\left((\Phi^2+\f^{2})\Lambda^{2}+\xi\right)}\right)^{\frac{\delta}{4\xi}},
%     \end{equation}
% $\delta = (\Phi_0^2-\Phi_\infty^2)$, and $\xi=\sqrt{4\dV^{2} \f^{2}+\delta^{2}}$. Note that we have not decided a priori whether $A_2>A_1$ or $A_2<A_1$. The way we have formulated the problem is agnostic to this choice. In either case, $\alpha$ will be entirely real and flipping $A_1$ and $A_2$ is equivalent to rotating the problem $90^\circ$ around $\e_3$. However, choosing $A_2>A_1$ for a growing inclusion prevents the need to calculate intermediate complex values. In the rest of this section we find it convenient to define $\alpha_0\equiv\hat{\alpha}(1)$ and to use the relation:
% \begin{equation}\label{eq:JStarCylinder}
% J^*_I = (\lambda^*)^2 = \frac{\varphi_0\alpha_0^2}{\Phi_0}\;,
% \end{equation}
% to calculate $\varphi_0$ where necessary. 

% For an inclusion made of a neo-hookean material, the total dimensionless elastic free energy of the inclusion-matrix system per unit depth in the $\e_3$ direction can be given as:
% \begin{equation}\label{eq:PsiCylinder}
%     \begin{split}
%         \bar{\Psi} =\;& \;\; \underbrace{\int_1^\infty \frac{\Phi}{\Phi_0}\Lambda\left[\frac{(\Phi_\infty^2-1)}{(\Phi+\Phi_\infty)^2}\left(\frac{\Phi_\infty^2}{\lambda^2\bar{\lambda}^2}-1\right)(\lambda-\bar{\lambda})^2 +\;\frac{\Phi_\infty^2}{\Phi^2}\left(\bar{\lambda}-\frac{1}{\bar{\lambda}}\right)^2 +\left(\lambda-\frac{1}{\lambda}\right)^2\right]\mathrm{d}\Lambda}_{\displaystyle\bar\Psi_M}\;\\
%         &+ (\lambda^*)^2\left[\left(\frac{\Phi_0}{\varphi_0}\right)^{\frac{1}{2}}-\left(\frac{\varphi_0}{\Phi_0}\right)^{\frac{1}{2}}\right]^2,
%     \end{split}
% \end{equation}
% where $\bar\Psi_M$ is the dimensionless elastic free energy of only the matrix per unit depth in the $\e_3$ direction. $\Phi_\infty$ can now be determined for a given  $\lambda^*$ and $\Phi_0$ by satisfying (\ref{eq:minimizationConditions}) via the single condition:
% \begin{equation}
%      \frac{\partial}{\partial\Phi_{\infty}}\bar{\Psi}(\lambda^*,\Phi_{0},\Phi_{\infty})=0\;.
% \end{equation}
% Finally, he Lagrangian pressure $q$ inside the inclusion can be determined by:
% \begin{equation}\label{eq:qCylinder}
%    \frac{q}{\mu} = -\frac{1}{2}\frac{\partial\bar\Psi_M}{\partial J^*_I} + \lambda^*\left[\frac{\partial\alpha_0}{\partial J^*_I}\left(\frac{\Phi_0}{\varphi_0}\right)^{\frac{1}{2}}+\;\left(\frac{\alpha_0}{J^*_I}-\;\frac{\partial\alpha_0}{\partial J^*_I}\right)\left(\frac{\varphi_0}{\Phi_0}\right)^{\frac{3}{2}}\right].
% \end{equation}
% Thus, we have fully determined the stress state inside the inclusion. 
% Unfortunately, because the authors were again unable to analytically solve the integral necessary to calculate $\bar\Psi_M$ this step was performed numerically to achieve the results in the following section. Maybe the reader will have the luck or skill necessary to attain fully analytical results. 
% \end{subequations}

==> Hold.tex <==
\section*{Appendix B: Derivation for General Ellipsoidal Equations as $\dV\to\infty$}
Now all that is left to fully describe the field is to find the $\Phi_\infty$ which minimizes the total free energy in the system $\Psi$. In order to perform the necessary volume and area integrals we find it convenient to parametrize the undeformed and deformed coordinates as:
\begin{subequations}
    \begin{equation}\label{eq:RefCoordsGEN}
       \X = A_1\Lambda\;\{\sin(v)\cos(u),\;\Phi_2\sin(v)\sin(u),\;\Phi_3\cos(v)\}\;,\;\mathrm{and}
    \end{equation}    
    \begin{equation}\label{eq:DefCoordsGEN}
        \x=A_1\alpha\;\{\sin(v)\cos(u),\;\varphi_2\sin(v)\sin(u),\;\varphi_3\cos(v)\}\;,
    \end{equation}  
\end{subequations}
respectively which satisfy (\ref{eq:xofXSum}). In this way any point in the inclusion-matrix system $\X\in\mathcal{D}^0$ can be identified by its undeformed radial parameter $\Lambda$ and its two angular parameters $u\in[0,2\pi)$ and $v\in[0,\pi)$. By taking the Jacobian of (\ref{eq:RefCoordsGEN}) with respect to $\{\Lambda,u,v\}$ we find that the volume integral over $\mathcal{D}^0$ in the reference cooridinates can be expressed as:
\begin{equation}\label{eq:volumeIntGEN}
    \int_{\mathcal{D}^0} \mathrm{dv}^0 = A_1^3\int_0^\infty\int_0^\pi\int_0^{2\pi} \left(\Phi_2\Phi_3\Lambda^2\sin(v)\Gamma\right)\mathrm{d}u\;\mathrm{d}v\;\mathrm{d}\Lambda\;,
\end{equation}
where for a spheroid in this parametrization $\Gamma = 1+\gamma_2 \sin^2(v)\sin^2(u)+\gamma_3 \cos^2(v)$. By taking the Jacobian of (\ref{eq:DefCoordsGEN}) with respect to $\{u,v\}$ and evaluating at $\Lambda=1$ we find that the surface integral over $\partial\mathcal{D}_I$ in the deformed coordinates can be expressed as:
\begin{equation}\label{eq:areaIntGEN}
    \int_{\partial\mathcal{D}_I} \mathrm{da} = \varphi_{02}\varphi_{03}\;a_1^2\int_0^\pi\int_0^{2\pi} \left(\sin(v)\sqrt{\sin^2(v)\cos^2(u)+\frac{1}{\varphi_{02}^2}\sin^2(v)\sin^2(u)+\frac{1}{\varphi_{03}^2}\cos^2(v)}\right)\mathrm{d}u\;\mathrm{d}v\;.
\end{equation}

Via (\ref{eq:FjkSimpInc}) we can find the first invariant of $\B$ inside the inclusion as $\dV\to\infty$:
\begin{subequations}
    \begin{equation}\label{eq:I1IncGEN}
        \lim_{\dV\to\infty}I_1=\left(\frac{\Phi_{02}\Phi_{03}}{\varphi_{\propto 2}\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\varphi_{\propto 2}^2\Phi_{03}}{\Phi_{02}^2\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\Phi_{02}\varphi_{\propto 3}^2}{\varphi_{\propto 2}\Phi_{03}^2}\right)^{\frac{2}{3}}
    \end{equation}
    and inserting (PAUSE) into (\ref{eq:FjkSimp}) and then using trigonometric identities to simplify, we can find the first invariant of $\B$ inside the matrix as $\dV\to\infty$:
    \begin{equation}\label{eq:I1MatGEN}
        \begin{split}
        \lim_{\dV\to\infty}I_1 \;= &\;\;\left(\frac{(\varphi_{\propto 2}^2-1)^2}{\varphi_{\propto 2}^2}\sin^2(v)\sin^2(u)\cos^2(u)+\frac{(\varphi_{\propto 3}^2-1)^2}{\varphi_{\propto 3}^2}\cos^2(v)\cos^2(u)\right.\\
        &\left.+\frac{(\varphi_{\propto 3}^2-\varphi_{\propto 2}^2)^2}{\varphi_{\propto 3}^2\varphi_{\propto 2}^2}\cos^2(v)\sin^2(u)\right)(\lambda-\bar{\lambda})^2\sin^2(v) +\left(2\bar{\lambda}^2+\frac{1}{\bar{\lambda}^4}\right), \;\forall\;\X\in\mathcal{D}^0_M\;.
        \end{split} 
    \end{equation}
\end{subequations}
We can use the expressions in (\ref{eq:I1IncGEN}) and (\ref{eq:I1MatGEN}) to find the elastic free energy per unit volume in the ungrown reference via (\ref{eq:NHFE}) and (\ref{eq:FERV}) and find the expression for the total elastic free energy in the inclusion-matrix system via (\ref{eq:totalFreeEnergyArb}) and (\ref{eq:areaIntGEN}) as:
\begin{equation} \label{eq:totalFreeEnergyGEN}
    \begin{split}
        \lim_{\dV\to\infty}\Psi =\;& \;\; \frac{\mu}{2}A_1^3\varphi_{\propto 2}\varphi_{\propto 3}\int_1^\infty\int_0^\pi\int_0^{2\pi} \Lambda^2\left[\left(\frac{(\varphi_{\propto 2}^2-1)^2}{\varphi_{\propto 2}^2}\sin^5(v)\sin^2(u)\cos^2(u)\right.\right.\\
        &\left.\left.+\frac{(\varphi_{\propto 3}^2-1)^2}{\varphi_{\propto 3}^2}\sin^3(v)\cos^2(v)\cos^2(u)+\frac{(\varphi_{\propto 3}^2-\varphi_{\propto 2}^2)^2}{\varphi_{\propto 3}^2\varphi_{\propto 2}^2}\sin^3(v)\cos^2(v)\sin^2(u)\right)(\lambda-\bar{\lambda})^2 \right.\;\\
        &\left.+\left(2\bar{\lambda^2}+\frac{1}{\bar{\lambda}^4}-3\right)\sin(v)\right]\mathrm{d}u\;\mathrm{d}v\;\mathrm{d}\Lambda\\
        &+ \frac{\mu}{2}(\lambda^*)^3\int_{\mathcal{D}^0_I}\left[\left(\frac{\Phi_{02}\Phi_{03}}{\varphi_{\propto 2}\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\varphi_{\propto 2}^2\Phi_{03}}{\Phi_{02}^2\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\Phi_{02}\varphi_{\propto 3}^2}{\varphi_{\propto 2}\Phi_{03}^2}\right)^{\frac{2}{3}}-3\right]\;\mathrm{dv}^0\;.
    \end{split}
\end{equation}
Because $I_1$ is uniform inside the inclusion, the second integral in this expression is trivial and we can simply multiply the integrand by $V^0$. The authors were able to analytically integrate the first integral over $u$ and $v$, but integration over $\Lambda$ is left as an exercise to the reader. Once the second integral is evaluated, and the first integral is integrated over $u$ and $v$ we can apply (\ref{eq:gammaSub}) where convenient and substitute the result into (\ref{eq:psibarDef}), yielding: 
\begin{equation}\label{eq:NDFEGEN}
    \begin{split}
        \lim_{\dV\to\infty}\bar\Psi =\;& \;\; \frac{\varphi_{\propto 2}\varphi_{\propto 3}}{\Phi_{02}\Phi_{03}}\int_1^\infty \Lambda^2\left[\frac{1}{5}\left(\frac{(\varphi_{\propto 2}^2-1)^2}{\varphi_{\propto 2}^2}+\frac{(\varphi_{\propto 3}^2-1)^2}{\varphi_{\propto 3}^2}+\frac{(\varphi_{\propto 3}^2-\varphi_{\propto 2}^2)^2}{\varphi_{\propto 3}^2\varphi_{\propto 2}^2}\right)(\lambda-\bar{\lambda})^2 \right.\;\\
        &\left.+3\left(2\bar{\lambda^2}+\frac{1}{\bar{\lambda}^4}-3\right)\right]\mathrm{d}\Lambda\\
        &+ (\lambda^*)^3 \left[\left(\frac{\Phi_{02}\Phi_{03}}{\varphi_{\propto 2}\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\varphi_{\propto 2}^2\Phi_{03}}{\Phi_{02}^2\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\Phi_{02}\varphi_{\propto 3}^2}{\varphi_{\propto 2}\Phi_{03}^2}\right)^{\frac{2}{3}}-3\right].
    \end{split}
\end{equation}
Again, notice that we did not assume a priori whether or not the ellipsoid was prolate or oblate. In the case of the oblate spheroid $\gamma>1$, and the logarithmic term becomes a inverse tangent term. In the case of the prolate spheroid $\gamma<1$ and the logarithmic term becomes a inverse hyperbolic tangent term. By expressing the result in this way we attain the general result for the spheroid, and the answer will always be fully real despite $\sqrt{-\gamma}$ being imaginary during the calculation of the term. This expression can now be evaluated numerically to satisfy (\ref{eq:minimizationConditions}) to find $\Phi_\infty$ for a given $\lambda^*$ and $\Phi_0$.
\begin{equation}
    \begin{split}
        \lim_{\dV\to\infty}\bar\Psi =\;& \;\; \underbrace{\frac{\dV}{\Phi_{02}\Phi_{03}}\left[\frac{1}{5}\left(\frac{(\varphi_{\propto 2}^2-1)^2}{\varphi_{\propto 2}^2}+\frac{(\varphi_{\propto 3}^2-1)^2}{\varphi_{\propto 3}^2}+\frac{(\varphi_{\propto 3}^2-\varphi_{\propto 2}^2)^2}{\varphi_{\propto 3}^2\varphi_{\propto 2}^2}\right)+5\right]}_{\displaystyle\lim_{\dV\to\infty}\bar\Psi_M}\\
        &+ \frac{\dV}{\Phi_{02}\Phi_{03}} \left[\left(\frac{\Phi_{02}\Phi_{03}}{\varphi_{\propto 2}\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\varphi_{\propto 2}^2\Phi_{03}}{\Phi_{02}^2\varphi_{\propto 3}}\right)^{\frac{2}{3}}+\left(\frac{\Phi_{02}\varphi_{\propto 3}^2}{\varphi_{\propto 2}\Phi_{03}^2}\right)^{\frac{2}{3}}-3\right].
    \end{split}
\end{equation}

\section{Isomorphic2}
In this limit, because we can imagine that the "cavity" which the inclusion occupies in the matrix began as a single point, it has no initial shape. Therefore we can choose any value of $\Phi_{02}$ and $\Phi_{03}$ in the the matrix, and in the limit where $\dV\to\infty$ the deformation fields \emph{must} be identical. In the inclusion on the other hand, since it has some reference shape which it maintains as it grows, $\Phi_{02}$ and $\Phi_{03}$ must still be chosen based on the relative values of the radii of the undeformed inclusion.

\subsection{Kinematics and the Isomorphic Aspect Ratio}
Since in this limit we may choose any value for $\Phi_{0J}$ inside the matrix we enforce that $\Phi_{0J}=\Phi_{\infty J}$ thus enforcing that $\Phi_J=\Phi_{\infty J}$ is constant for all $\X\in\mathcal{D}^0_M$. Assuming a generalized set of ellipses of the form in (\ref{eq:PhiGj}), this implies that as $\dV\to\infty$, we may choose $\Phi'_2=0$ and $\Phi'_3=0$  and by extension, because $\Phi_J>0$ and inside the matrix $\Lambda>1$, $\gamma_2=0$ and $\gamma_3=0$ for all $\X\in\mathcal{D}^0_M$. Thus, the incompressibility conditions which must be satisfied for our kinematic assumptions (\ref{eq:IncompGam2Gen}) and (\ref{eq:IncompGam3Gen}) (or (\ref{eq:IncompGam22D}) for the case of an elliptic cylinder under plane isotropic growth) imply that $\displaystyle{\lim_{\dV\to\infty}\beta_2=0}$ and $\displaystyle{\lim_{\dV\to\infty}\beta_3=0}$ and by extension, because $\varphi_J>0$ and inside the matrix $\alpha>0$, $\displaystyle{\lim_{\dV\to\infty}\varphi'_2=0}$ and $\displaystyle{\lim_{\dV\to\infty}\varphi'_3=0}$ for all $\X\in\mathcal{D}^0_M$. This directly implies that given our kinematic assumptions as  $\displaystyle{\lim_{\dV\to\infty}\varphi_2}$ and $\displaystyle{\lim_{\dV\to\infty}\varphi_3}$ are constant in $\Lambda$ for all $\X\in\mathcal{D}^0_M$. Because the deformation must vanish as $\Lambda\to\infty$ (far away from the inclusion) this implies $\displaystyle{\lim_{\Lambda\to\infty}\hat{\varphi_J}=\lim_{\Lambda\to\infty}\hat{\Phi_J}=\Phi_{0J}}$. Thus, given our kinematic assumptions, in the $\displaystyle{\lim_{\Lambda\to\infty}\Chi}$ the field becomes equivalent to a field in the limit of where $V^0/V^*\to0$ described by:
\begin{subequations}
\begin{equation}
    \hat\Phi_J(\Lambda) = 
    \begin{cases}
    \Phi_{0J}, & 0<\Lambda< 1 \\
    \varphi_{\propto J}, & \Lambda>1\;,
    \end{cases}
\end{equation}
\begin{equation}
    \hat\varphi_J(\Lambda) = \varphi_{\propto J}, \;\; \forall\; \Lambda\;,
\end{equation}
and by extension from (\ref{eq:TotIncompInc}) and (\ref{eq:TotIncompMat}),
\begin{equation}\label{eq:isomorphicAlphaGen}
    \hat\alpha(\Lambda) = 
    \begin{cases}
    \displaystyle\lambda^*\left(\frac{\Phi_{02}\Phi_{03}}{\varphi_{\propto 2}\varphi_{\propto 3}}\right)^{\frac{1}{3}}\Lambda\;, & 0<\Lambda< 1 \\
    \displaystyle\left(\Lambda^3+\frac{\dV}{\varphi_{\propto 2}\varphi_{\propto 3}}\right)^{\frac{1}{3}}, & \Lambda>1\;,
    \end{cases}
\end{equation}
\end{subequations}
where we define $\varphi_{\propto 2}\equiv\displaystyle{\lim_{\dV\to\infty}\varphi_2}$ and $\varphi_{\propto 3}\equiv\displaystyle{\lim_{\dV\to\infty}\varphi_3}$ as the isomorphic aspect ratios, because in this \emph{isomorphic limit} the shape of the deformed inclusion arrives at some constant shape as $\dV\to\infty$. For a spheroid (\ref{eq:isomorphicAlphaGen}) simplifies to:
\begin{equation}
    \hat\alpha(\Lambda) = 
    \begin{cases}
    \displaystyle\lambda^*\left(\frac{\Phi_{0}}{\varphi_{\propto }}\right)^{\frac{1}{3}}\Lambda\;, & 0<\Lambda< 1 \\
    \displaystyle\left(\Lambda^3+\frac{\dV}{\varphi_{\propto }}\right)^{\frac{1}{3}}, & \Lambda>1\;.
    \end{cases}
\end{equation}
Note that this can also be found by taking the limit of (\ref{eq:alphaMatSpheroid}) as $\dV\to\infty$ corroborating this result. From (\ref{eq:TotIncompInc2D}) and (\ref{eq:TotIncompMat2D}), for an elliptic cylinder under plane isotropic growth or contraction (\ref{eq:isomorphicAlphaGen}) becomes:
\begin{equation}
    \hat\alpha(\Lambda) = 
    \begin{cases}
    \displaystyle\lambda^*\left(\frac{\Phi_{0}}{\varphi_{\propto }}\right)^{\frac{1}{2}}\Lambda\;, & 0<\Lambda< 1 \\
    \displaystyle\left(\Lambda^2+\frac{\dV}{\varphi_{\propto }}\right)^{\frac{1}{2}}, & \Lambda>1\;.
    \end{cases}
\end{equation}
Again, note that this can also be found by taking the limit of (\ref{eq:alphaexpanded2D}) as $\dV\to\infty$ corroborating this result.

\subsection{The Isomorphic Stress State}
